Dynamic Spectral Clustering with Provable Approximation Guarantee

This paper studies clustering algorithms for dynamically evolving graphs $\{G_t\}$, in which new edges (and potential new vertices) are added into a graph, and the underlying cluster structure of the graph can gradually change. The paper proves that, under some mild condition on the cluster-structure, the clusters of the final graph $G_T$ of $n_T$ vertices at time $T$ can be well approximated by a dynamic variant of the spectral clustering algorithm. The algorithm runs in amortised update time $O(1)$ and query time $o(n_T)$. Experimental studies on both synthetic and real-world datasets further confirm the practicality of our designed algorithm.

==> algorithms/spectral_clustering.tex <==
\begin{algorithm}[ht]
\caption{\textsf{SpectralClustering}}\label{alg:spectralclustering}
\KwData{$G=(V,E)$, $k\in\mathbb{N}$}
\KwResult{A partitioning $P_1, \ldots, P_k$}
Compute $f_1, \ldots, f_k$ of $\mathcal{L}_G$\; 
\For{$u \in V$}{
$F(u) \leftarrow \frac{1}{\sqrt{d_u}}\cdot (f_1(u),\ldots, f_k(u))^{\intercal}$\;
}
$P_1, \ldots, P_k \leftarrow k\mbox{-means} (\{F(u)\}_{u\in V}, k)$\;
\Return{$P_1, \ldots, P_k$}
\end{algorithm}
